Algorithms for Algebraic Path Properties in Concurrent Systems of Constant Treewidth Components

We study algorithmic questions for concurrent systems where the transitions are labeled from a complete, closed semiring, and path properties are algebraic with semiring operations. The algebraic path properties can model dataflow analysis problems, the shortest path problem, and many other natural problems that arise in program analysis. We consider that each component of the concurrent system is a graph with constant treewidth, a property satisfied by the controlflow graphs of most programs. We allow for multiple possible queries, which arise naturally in demand driven dataflow analysis. The study of multiple queries allows us to consider the tradeoff between the resource usage of the one-time preprocessing and for each individual query. The traditional approach constructs the product graph of all components and applies the best-known graph algorithm on the product. In this approach, even the answer to a single query requires the transitive closure, which provides no room for tradeoff between preprocessing and query time. Our main contributions are algorithms that significantly improve the worst-case running time of the traditional approach, and provide various tradeoffs depending on the number of queries. For example, in a concurrent system of two components, the traditional approach requires hexic time in the worst case for answering one query as well as computing the transitive closure, whereas we show that with one-time preprocessing in almost cubic time, each subsequent query can be answered in at most linear time, and even the transitive closure can be computed in almost quartic time. Furthermore, we establish conditional optimality results showing that the worst-case running time of our algorithms cannot be improved without achieving major breakthroughs in graph algorithms.

==> intro_bk.tex <==
\section{Introduction\label{sec:intro}}

In this work we consider concurrent finite-state systems where each 
component system is a constant-treewidth graph, 
and the algorithmic question is to determine algebraic path properties between pairs of nodes in the system.
Our main contributions are algorithms which significantly improve
the worst-case running time of the previous known algorithms.
We establish conditional optimality results for some of our algorithms 
in the sense that they cannot be improved without achieving major 
breakthrough in the algorithmic study of graph problems.
We also present experimental results which show that our algorithms perform
favorably for several real-world benchmarks.
%%well in practice. 



\smallskip\noindent{\em Concurrency and algorithmic approaches.}
The analysis of concurrent systems is one of the fundamental problems in 
computer science in general, and programming languages in particular.
A finite-state concurrent system consists of several components, 
each of which is a finite-state graph, and the whole system is a composition 
of the components.
Since errors in concurrent systems are hard to reproduce by simulations 
due to combinatorial explosion in the number of interleavings, 
formal methods are necessary to analyze such systems. 
In the heart of the formal approaches are graph algorithms, which 
provide the basic search procedures for the problem.
The basic graph algorithmic approach is to construct the product graph 
(i.e., the product of the component systems) and then apply the 
best-known graph algorithms on the product graph.
While there are many practical approaches for the analysis of concurrent systems,
a fundamental theoretical question is whether special properties of graphs that 
arise in analysis of programs can be exploited to develop faster algorithms
as compared to the baseline approach. 


\smallskip\noindent{\em Special graph properties for programs.}
A very well-studied notion in graph theory is the concept of {\em treewidth} 
of a graph, which is a measure of how similar a graph is to a tree 
(a graph has treewidth~1 precisely if it is a tree)~\cite{Robertson84}. 
The treewidth of a graph is defined based on a {\em tree decomposition} of 
the graph~\cite{Halin76}, see Section~\ref{sec:definitions} for a formal 
definition.
On one hand the treewidth property provides a mathematically elegant way 
to study graphs, and on the other hand there are many classes of graphs which 
arise in practice and have constant treewidth. 
The most important example is that the control flow graph for goto-free 
programs for many programming languages are of constant 
treewidth~\cite{Thorup98}, 
which has also been demonstrated experimentally even at the presence of gotos~
(\cite{Gustedt02,Burgstaller04}).


\smallskip\noindent{\em Algebraic path properties.}
To specify properties of traces of concurrent systems we consider a very 
general framework, where edges of the system are labeled from a complete, 
closed semiring (which subsumes bounded and finite distributive semirings), 
and we refer to the labels of the edges as weights. 
For a given path, the weight of the path is the semiring product of the weights
on the edges of the path, and to choose among different paths we use the 
semiring plus operator. 
For example, (i)~the Boolean semiring (with semiring product as AND, and 
semiring plus as OR) expresses the reachability property; 
(ii)~the tropical semiring (with real-edge weights, semiring product as 
standard sum, and semiring plus as minimum) expresses the shortest path 
property; and (iii)~with letter labels on edges, semiring product as string 
concatenation and semiring plus as union we can express the regular expression 
of reaching from one node to another.
The algebraic path properties expressed in our framework subsumes the dataflow analysis of the
IFDS/IDE frameworks~\cite{Reps95,Sagiv96} in the intraprocedural setting,
which consider compositions of distributive dataflow functions, and meet over all paths as the semiring plus operator.
Since IFDS/IDE are subsumed in our framework, the large and important class of 
dataflow analysis problems that can be expressed in the IFDS/IDE frameworks 
can also be expressed in our framework, when we focus our interest to the intraprocedural analysis.

\smallskip\noindent{\em Expressiveness of algebraic path properties.}
The algebraic path properties provide a very rich and expressive framework, 
and we discuss two instances of them.
\begin{compactenum}

\item {\em Weighted shortest path.} 
The weighted shortest path (which can be expressed
on the tropical semiring) can model a variety of 
properties~\cite{Reps07,Reps05,Lal08b}. 
For example, the edge weights (positive and negative) can express energy 
consumptions, and the shortest path problem asks for the least energy 
consuming path.
Another important quantitative property is the \emph{mean-payoff} property, 
where each edge weight represents a reward or cost, and the problem asks for 
a path that minimizes the average of the weights along a path. 
Many quantitative properties of relevance for program analysis (e.g., to 
express performance or resource consumption) can be modeled as mean-payoff 
properties~\cite{Chatterjee15B,CHR13}.
It follows from the results of~\cite{K78,L76} that for finite-state graphs,
the mean-payoff property can be computed by solving the weighted shortest path 
problem. 

\item {\em Regular expressions.}
Consider the case that each edge label represents an observable. 
Then the regular expression to reach from one node to another represent all the 
sequences of observable actions that lead from the start node to the target.
It was shown in~\cite{Cerny15} that several problems for concurrency analysis
can be modeled as the language inclusion problem given the regular expression.
For example, the regular expression can represent a set of error traces
(instead of a single error trace), and can help in accelerating the 
abstraction-refinement loop by ruling out several traces instead of a 
single one~\cite{Cerny15}.
Hence computing regular expression is another important algebraic path 
property.

\end{compactenum}




\smallskip\noindent{\em The algorithmic problem.}
In graph theoretic parlance, graph algorithms typically consider two types of 
queries: (i)~a \emph{pair query} that given nodes $\ov{u}$ and $\ov{v}$ 
(called $(\ov{u},\ov{v})$-pair query) asks for the algebraic path property 
from $\ov{u}$ to $\ov{v}$; and 
(ii)~a \emph{single-source} query that given a node $\ov{u}$ asks for the 
answer of $(\ov{u},\ov{v})$-pair queries for all nodes $\ov{v}$.
Since we consider the concurrent setting, in addition to the classical pair 
and single-source queries, we also consider {\em partial} queries. 
Given a concurrent system with $k$ components, a node in the product graph 
is a tuple of $k$ component nodes. 
A \emph{partial} node in the product only specifies nodes of a nonempty 
strict subset of all the components.
Our work also considers partial pair and partial single-source queries, 
where the input nodes are partial nodes.
Queries on partial nodes are very natural, as they capture 
properties between local locations in a component, 
that are shaped by global paths in the whole concurrent system.
For example, constant propagation and dead code elimination are local properties in a program,
but their analysis requires analyzing the concurrent system as a whole.
%The main purpose to consider partial queries is as follows: consider a 
%concurrent system with two components, and if we are interested to know 
%whether a node $u_1$ in the first component is reachable from another node 
%$v_1$ of the component, irrespective of the start and end nodes
%of the other component, then this is modeled succinctly as a partial 
%pair query. 

%Say that most of these works offer no theoretical improvement on the on-demand queries
\smallskip\noindent{\em Preprocess vs query.}
A topic of widespread interest in the programming languages community is that of on-demand analysis
~\cite{WayneA78,Zadeck84,Horwitz95,Duesterwald95,Reps95b,Sagiv96,Reps97,Yuan97,Naeem10,CIPG15}.
Such analysis has several advantages, such as (quoting from~\cite{Horwitz95,Reps97})
(i)~narrowing down the focus to specific points of interest,
(ii)~narrowing down the focus to specific dataflow facts of interest,
(iii)~reducing work in preliminary phases,
(iv)~sidestepping incremental updating problems, and
(v)~offering demand analysis as a user-level operation.
%\begin{compactenum}
%\item Narrowing down the focus to specific points of interest
%\item Narrowing down the focus to specific dataflow facts of interest
%\item Reducing work in preliminary phases
%\item Sidestepping incremental updating problems
%\item Offering demand analysis as a user-level operation
%\end{compactenum}
For example, in alias analysis, the question is whether two pointers may point to the same 
object, which is by definition modeled as a question between a pair of nodes.
Similarly, e.g., in constant propagation a relevant question is whether 
some variable remains constant between a pair of control flow locations.
The problem of on-demand analysis allows us to distinguish between a single preprocessing phase 
(one time computation), and a subsequent query phase, where queries are answered on demand.
The two extremes of the preprocessing and query phase are as follows:
(i)~\emph{complete preprocessing} (aka \emph{transitive closure} computation) 
where the result is precomputed for every possible query, and hence queries are 
answered by simple table lookup; and (ii)~\emph{no preprocessing} where no 
preprocessing is done, and every query requires a new computation.
However, in general there can be a tradeoff between the preprocessing and 
query computation.
%Write that on demand offer practical guarantee, and the theoretical is only for all queries.
Most of the existing works for on-demand analysis do not make a formal distinction between preprocessing and query phases,
as the provided complexities only guarantee the \emph{same-worst-case-cost property},
namely that the total time for handling any sequence of queries is no worse than the complete preprocessing.
Hence most existing tradeoffs are practical, without any theoretical guarantees.


\smallskip\noindent{\em Previous results.} 
In this work we consider finite-state concurrent systems, where each 
component graph has constant treewidth, and the trace properties are specified as algebraic path properties. 
Our framework can model a large class of problems: typically the 
control flow graphs of programs have constant treewidth~\cite{Thorup98,Gustedt02,Burgstaller04}, 
and if there is a constant number of synchronization variables with constant-size domains, 
then each component graph has constant treewidth. 
Note that this imposes no practical restrictions, as typically synchronization variables,
such as locks, mutexes and condition variables have small (even binary) domains (e.g. locked/unlocked state).
The best-known graph algorithm for the algebraic path property problem is the 
classical Warshall-Floyd-Kleene~\cite{Lehmann77,Floyd62,Warshall62,Kleene56} style dynamic programming, which requires cubic time.
Two well-known special cases of the algebraic path problem are those of computing the shortest path from a source to a sink node in a weighted graph,
and computing the regular expression from a source to a sink node in an automaton whose edges are labeled with letters from a finite alphabet.
In the first case, the best-known algorithm is the Bellman-Ford algorithm with
time complexity $O(n\cdot  m)$ (where $n$ is the number of vertices and $m$ is
the number of edges, and since $m$ can be $n^2$, the worst-case bound is $O(n^3)$).
In the second case, the well-known construction of Kleene's~\cite{Kleene56} theorem requires cubic time.
The only existing algorithmic approach for the problem we consider is to first 
construct the product graph (thus if each component graph has size $n$, and
there are $k$ components, then the product graph has size $O(n^k)$), and then 
apply the best-known graph algorithm (thus the overall time complexity is 
$O(n^{3\cdot k})$).
Hence for the important special case of two components we obtain a hexic-time (i.e., $O(n^6)$) algorithm.
Moreover, for algebraic path properties (even for the special case of shortest 
path) the current best-known algorithms for one pair query (or one 
single-source query) computes the entire transitive closure. 
Hence the existing approach does not allow a tradeoff of preprocessing and
query as even for one query the entire transitive closure is computed.


\begin{table*}
\centering
\begin{ThreePartTable}
\small
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c||c|c||c|c|c|c|}
\hline
& \multicolumn{2}{c||}{Preprocess} & \multicolumn{4}{c|}{Query time}\\
\cline{2-7}
& Time & Space \tnotex{tn:space} & Single-source & Pair & Partial single-source & Partial-pair\\
\hline
\hline
Previous results~\cite{Lehmann77,Floyd62,Warshall62,Kleene56} & $O(n^6)$ & $O(n^4)$ & $O(n^2)$ & $O(1)$ & $O(n^2)$ & $O(1)$\\
\hline
%\hline
%No preprocess~\cite{Lehmann77,Floyd62,Warshall62,Kleene56} & $-$ & $O(n^4)$ & $O(n^6)$ & $O(n^6)$ & $O(n^6)$\\
{\bf Our result \cref{cor:ld}}~$(\eps>0)$ & $\mathbf{O(n^{3})}$ & $\mathbf{O(n^{2+\eps})}$ & $\mathbf{O(n^{2+\eps})}$ & $\mathbf{O(n^{2})}$ & $\mathbf{O(n^{2+\eps})}$ & $\mathbf{O(n^{2})}$\\
\hline
{\bf Our result \cref{them:concurrent}}~$(\eps>0)$  & $\mathbf{O(n^{3+\eps})}$ & $\mathbf{O(n^3)}$ & $\mathbf{O(n^{2+\eps})}$ & $\mathbf{O(n)}$ & $\mathbf{O(n^2)}$ & $\mathbf{O(1)}$\\
\hline
{\bf Our result \cref{cor:closure}}~$(\eps>0)$  & $\mathbf{O(n^{4+\eps})}$ & $\mathbf{O(n^4)}$ & $\mathbf{O(n^{2})}$ & $\mathbf{O(1)}$ & $\mathbf{O(n^2)}$ & $\mathbf{O(1)}$\\
%{\bf \cref{them:tradeoff}}~$(\eps\in [0,\Epsbound])$ & $\mathbf{O(n^{3+\eps})}$ & $\mathbf{O(n^{2.4})}$ & $\mathbf{O(n^{2.4})}$ & $\mathbf{O(n^{2-\eps})}$ & $\mathbf{O(n^{2-3\cdot \eps})}$\\
\hline
\end{tabular}
\caption{The algorithmic complexity for computing algebraic path queries wrt a closed, complete semiring on a concurrent graph 
$G$ which is the product of two constant-treewidth graphs $G_1$, $G_2$, with $n$ nodes each.}
\label{tab:intro1}
\begin{tablenotes}
\item[a] \label{tn:space} Space complexity is measured as the total space usage in preprocessing and one query.
\end{tablenotes}
\end{ThreePartTable}
\end{table*}


\input{fig_outline}


\smallskip\noindent{\em Our contributions.} 
Our main contributions are improved algorithmic upper bounds,
proving several optimality results of our algorithms, and experimental 
results.
Below all the complexity measures (time and space) are in the number of basic 
machine operations and number of semiring operations. 
We elaborate our contributions below.

\begin{compactenum}
\item {\em Improved upper bounds.}
%%The results are stated for a data-structure that operates on input
%%of a concurrent graph $G$ that consists of $k$ components.
%%The data-structure has a preprocessing phase, follows by a query phase
%%in which it answers algebraic path queries.
We present improved upper bounds both for general $k$ components,
and the important special case of two components.


\begin{compactitem}
\item \emph{General case.} 
We show that for $k\geq 3$ components with $n$ nodes each, with 
$O(n^{3\cdot (k-1)})$ preprocessing time, we can answer 
(i)~single-source queries in $O(n^{2\cdot (k-1)})$ time, 
(ii)~pair query in $O(n^{k-1})$ time, 
(iii)~partial single-source queries in $O(n^k)$ time, and 
(iv)~partial pair queries in $O(1)$ time; 
and our space requirement is $O(n^{2\cdot k -1})$.
In contrast, the existing methods~\cite{Lehmann77,Floyd62,Warshall62,Kleene56}
that compute the transitive closure of the graph require 
$O(n^{3\cdot k})$ time and $O(n^{2\cdot k})$ space.
 
\item \emph{Two components.} 
For the important special case of two threads, the existing methods 
require $O(n^6)$ time and $O(n^4)$ space even for one query.
In contrast, we establish a variety of tradeoffs between preprocessing and 
query times, and the best choice depends on the number of queries.
In particular, for any fixed $\eps>0$, we establish three results (\cref{sec:concurrent}): 

\smallskip\noindent{\em Three results.}
First, we show (in~\cref{cor:ld}) that with 
$O(n^3)$ preprocessing time and using $O(n^{2+\eps})$ space, we can answer
single-source queries in $O(n^{2+\eps})$ time, and 
pair and partial pair queries require $O(n^2)$ time.
Second, we show (in~\cref{them:concurrent}) that 
with $O(n^{3+\eps})$ preprocessing time and using $O(n^3)$ space,
we can answer the pair and the partial pair query in time 
$O(n)$ and $O(1)$, respectively.
Third, we show (in~\cref{cor:closure}) that 
the transitive closure can be computed using $O(n^{4+\eps})$ preprocessing time 
and $O(n^{4})$ space, after which single-source queries require $O(n^2)$ time, 
and pair and partial pair queries require $O(1)$ time
(i.e., all queries require linear time in the size of the output).

\smallskip\noindent{\em Tradeoff.}
Our result provides various tradeoffs:
The first result is best for answering $O(n^{1+\eps})$ pair and partial pair 
queries;
the second result is best for answering between $\Omega(n^{1+\eps})$ and  
$O(n^{3+\eps})$ pair queries, and $\Omega(n^{1+\eps})$ partial pair queries; 
and the third result is best when answering $\Omega(n^{3+\eps})$ pair queries.
Observe that the transitive closure computation is preferred when the number 
of queries is large, in sharp contrast to the existing methods that compute 
the transitive closure even for a single query.
Our results are summarized in~\cref{tab:intro1} and the tradeoff is 
pictorially illustrated in~\cref{fig:outline}.
\end{compactitem}





\item {\em Optimality of our results.}
Given our significant improvements for the case of two components, a very 
natural question is whether the algorithms can be improved further. 
While presenting matching  bounds for polynomial-time graph algorithms 
to establish optimality is very rare in the whole of computer science, 
we present \emph{conditional lower bounds} to show that the total of 
preprocessing and query time of our results cannot be improved without
achieving a major breakthrough in graph algorithms.

\begin{compactitem}

\item {\em Almost optimality.} 
First, note that for the first result (obtained from~\cref{cor:ld})
our space usage and single-source query time are arbitrarily close to 
optimal, as both the input and the output have size $\Theta(n^2)$.
Moreover, the result is achieved with preprocessing time less than 
$\Omega(n^4)$, which is a lower bound to compute the transitive closure 
which has $n^4$ entries.
Furthermore, for our third result (obtained from~\cref{cor:closure}) 
the $O(n^{4 + \eps})$ preprocessing time is arbitrarily close to optimal, and the $O(n^4)$ preprocessing 
space is indeed optimal, 
as the transitive closure computes the distance among all $n^4$ pairs of 
nodes (which requires $\Omega(n^4)$ time and space).

\item {\em Conditional lower bound.}
In recent years, the conditional lower bound problem has received
a lot of attention in complexity theory, where under the assumption that 
certain problems (such as matrix multiplication, all-pairs shortest path)
cannot be solved faster, lower bounds for other problems (such as 
dynamic graph algorithms) are obtained~\cite{AW14,AWY15,HKNS15}.
The current best-known algorithm for algebraic path properties for general 
(not constant-treewidth) graphs is cubic in the number of nodes.
Even for the special case of shortest paths with positive and negative 
weights, the best-known algorithm (which has not been improved over five 
decades) is $O(n\cdot  m)$, where $m$ is the number of edges. 
Since $m$ can be $\Omega(n^2)$, the current best-known worst-case complexity 
is cubic in the number of nodes.
We show that pair queries takes longer to solve in a concurrent graph of two 
constant-treewidth graphs, with $n$ nodes each, than in general graphs with 
$n$ nodes.
This implies that improving the $O(n^3)$ combined preprocessing and query time over our result (from~\cref{cor:ld}) for answering $r$ queries, for $r\leq O(n)$, 
would yield the same improvement over the $O(n^3)$ time for answering $r$ pair queries in general 
graphs. 
Note that improving the $O(n^3)$ time for general graphs, even for a single 
pair query, would be a major breakthrough. 
In other words, the combination of our preprocessing and query time 
(from~\cref{cor:ld}) cannot be improved without improving the long standing 
cubic (in the number of nodes) bound for the shortest path and the algebraic 
path problems in general graphs.
Furthermore, this also implies that our result (from \cref{them:concurrent}) 
cannot be improved much further even for $n^2$ queries,
as the combined time for preprocessing and answering $n^2$ 
queries is $O(n^{3+\epsilon})$ using \cref{them:concurrent} while
the existing bound is $O(n^3)$ for general graphs. 
%Note that in general graphs with $n$ nodes there are at most $n^2$ distinct 
%pair queries. 
\end{compactitem}


\item {\em Experimental results.}
{\bf TO BE FILLED.}

\end{compactenum}



\smallskip\noindent{\em Technical contributions.}
The results of this paper rely on several technical contributions.
\begin{compactenum}

\item \emph{Upper bounds}.
Our upper bounds depend on a series of technical results.
\begin{compactenum}
\item 
The first key result for our upper bounds is an algorithm 
for constructing a \emph{strongly balanced} tree-decomposition $T$.
A tree is called $(\beta, \gamma)$-balanced if for every node $u$ and every descendant $v$ of $u$
that appears  $\gamma$ levels below,
the size of the subtree of $T$ rooted at $v$ is at most a $\beta$ fraction of the size
of the subtree of $T$ rooted at $u$.
For any fixed $\delta>0$ and $\lambda\in \Nats$ with $\lambda\geq 2$,
let $\beta=\Balfactor$ and $\gamma=\Levelfactor$.
We show that a $(\beta,\gamma)$-balanced tree decomposition of a constant-treewidth graph 
with $n$ nodes can be constructed in $O(n\cdot \log n)$ time and $O(n)$ space.
To our knowledge, this is the first algorithm that constructs a tree decomposition 
with such a strong notion of balance.
This  property is crucial for achieving the resource bounds of our algorithms
for algebraic path queries.
The construction is presented in \cref{sec:prelim_tree_dec}.
\item 
Given a concurrent graph $G$ obtained from $k$ constant-treewidth graphs $G_i$, 
we show how a tree-decomposition of $G$ can be constructed from the strongly balanced 
tree-decompositions $T_i$ of the components $G_i$, in time that is linear in the size of the output.
We note that $G$ can have large treewidth, and thus determining the treewidth of $G$ can be computationaly 
expensive.
Instead, our construction avoids computing the treewidth of $G$, and 
directly constructs a tree-decomposition of $G$ from the strongly balanced
component tree decompositions. %%%that is optimal in the worst case. 
This construction is presented in \cref{sec:product_tree_dec}.
\item
Given the above tree-decomposition algorithm for concurrent graphs $G$,
in \cref{sec:concurrent} we present the algorithms for handling algebraic path queries.
In particular, we introduce the \emph{partial expansion} $\PNode{G}$ of $G$ for additionally handling partial queries,
and describe the algorithms for preprocessing and querying $\PNode{G}$ in the claimed time and space bounds.
\end{compactenum}
\item \emph{Lower bound}.
Given an arbitrary graph $G$ (not of constant treewidth) of $n$ nodes, we show how to construct
a constant-treewidth graph $G''$ of $2\cdot n$ nodes, and a graph $G'$ that is 
the product of $G''$ with itself, such that algebraic path queries in $G$ coincide with 
such queries in $G'$.
The construction of $G''$ itself takes linear time and the product construction  
is quadratic time.
The conditional optimality of our algorithms follows, as improvement over our algorithms 
must achieve the same improvement for algebraic path properties on arbitrary graphs.
\end{compactenum}
All our algorithms are simple to implement and provided as pseudocode in \cref{sec:algorithms}.



\subsection{Related Works}


\smallskip\noindent{\em Treewidth of graphs.}
The notion of treewidth for graphs as an elegant mathematical tool
to analyze graphs was introduced in~\cite{Robertson84}.
The significance of constant treewidth in graph theory is huge 
mainly because several problems on graphs become complexity-wise easier.
Given a tree decomposition of a graph with low treewidth $t$, 
many NP-complete problems for arbitrary graphs can be solved in time polynomial 
in the size of the graph, but exponential in $t$~\cite{Arnborg89,Bern1987216,Bodlaender88,Bodlaender93,Bodlaender05}. 
Even for problems that can be solved in polynomial time, 
faster algorithms can be obtained for low treewidth graphs,
for example, for the distance problem~\cite{Chaudhuri95}.
The constant-treewidth property of graphs has also been used in the context
of logic: Monadic Second Order (MSO) logic is a very expressive logic, and a 
celebrated result of~\cite{Courcelle91} showed that for constant-treewidth graphs the 
decision questions for MSO can be solved in polynomial time; and 
the result of~\cite{Elberfeld10} shows that this can even be achieved in deterministic
log-space.
Various other models (such as probabilistic models of Markov decision processes
and games played on graphs for synthesis) with the constant-treewidth restriction 
have also been considered~\cite{CL13,Obdrzalek03}.
The problem of computing a balanced tree decomposition for a constant treewidth 
graph was considered in~\cite{Reed92}.
More importantly, in the context of programming languages, it was shown by~\cite{Thorup98}
that the control flow graphs of goto-free programs from many programming languages have 
constant treewidth.
This theoretical result was subsequently followed up in several practical approaches,
and although in the presence of gotos the treewidth is not bounded,
it has been shown that programs in several programming languages have low treewidth in practice
(\cite{Gustedt02,Burgstaller04}).
The constant-treewidth property of graphs has been used to develop faster algorithms
for sequential interprocedural analysis~\cite{CIPG15},
%%for obtaining tractable solutions to the register allocation problem~\cite{Thorup98,Bodlaende98},
and on the analysis of automata with auxiliary storage (e.g., stacks and queues)~\cite{Madhusudan11}.
%In~\cite{CIPG15} the constant-treewidth property is exploited for interprocedural
%analysis but without concurrency, whereas we consider intraprocedural analysis 
%with concurrency. 
The techniques of~\cite{CIPG15} do not extend to the concurrent setting because 
even though the component graphs have constant treewidth, the graph which is 
product of the components has treewidth that depends on the number of nodes.
Thus none of the previous works exploit the constant-treewidth property
for faster algorithms in the concurrent setting. 


\smallskip\noindent{\em Concurrent system analysis.}
The problem of concurrent system analysis has been considered in several 
works, both for intraprocedural as well context-bounded interprocedural
analysis~\cite{Harel97,Alur99,Farzan13,Qadeer05,Bouajjani05,LaTorre08, Lal08,Lal09}, 
and many practical tools have been developed as well~\cite{Qadeer05, Lal09,Suwimonteerabuth08,Lal12}.
In this work we focus on the intraprocedural analysis with constant-treewidth
graphs, and present algorithms with better asymptotic complexity.
None of the previous works consider the constant-treewidth property, nor the 
improve the asymptotic complexity of the basic algorithm for the algebraic 
path property problem.



==> recurrence.tex <==
\section{Recurrence}\label{sec:recurrence}



==> tradeoff.tex <==
\section{Preprocessing-Query Time Tradeoff for Two Graphs}\label{sec:tradeoff}
In this section, we focus on the case where the concurrent graph $G$
of two constant-treewidth graphs $G_1$, $G_2$.
We modify the data-structure $\ConcurAP$ presented in the last section
such that for any fixed $\eps\in[0,\Epsbound]$, we obtain a data-structure $\ConcurAP^{\eps}$
that has $O(n^{3+\eps})$ preprocessing time and $O(n^{2-\eps})$ pair, and $O(n^{2-3\cdot \eps})$ partial pair query time.
That is, $\ConcurAP^{\eps}$ trades preprocessing for query time.
Additionally, $\ConcurAP^{\eps}$ uses at all times $O(n^{2.4})$ space.
In the next section, we establish that $\ConcurAP^{0}$ is optimal in a certain sense.


\smallskip\noindent{\bf A warmup modification for $\ConcurAP^{0}$.}
We first describe a simple modification that leads to $O(n^3)$ preprocessing and $O(n^2)$ pair query time.
This is achieved by modifying \cref{item:ancestors} of $\Concpreprocessalgo$.
Recall that in this step, for every node $u$, the maps
$\From_{u}, \To_{u}: \AncestV{\PNode{V}}_{\PNode{T}}(\PNode{\Bag}_u) \to \Sigma$
store the distance between $u$ and every partial node $\PNode{v}\in \AncestV{\PNode{V}}_{\PNode{T}}(\PNode{\Bag}_u)$.
Instead, now the partial nodes $\PNode{v}$ are taken to be $\PNode{v}\in \PNode{\Bag}_u\cup \PNode{\Bag}'$,
where $\PNode{\Bag}'$ is the parent of $\PNode{\Bag}_u$ in $\PNode{T}$.
In words, instead of storing the distance between $u$ and partial nodes that appear in $\PNode{\Bag}_u$ and its ancestors,
we only store this distance for partial nodes that appear in $\PNode{\Bag}_u$ and its parent.
This is done by executing an all-pairs algebraic paths computation in $\PNode{G}\restr{\PNode{\Bag}\cup \PNode{\Bag}'}$
for every bag $\PNode{\Bag}$ and its parent $\PNode{\Bag}'$,
with the weight function $\Weightmap:\PNode{\Bag}\cup \PNode{\Bag}'\to \Sigma$ obtained from the maps $\Fwd$ and $\Bwd$
constructed in \cref{item:ld} of $\Concpreprocessalgo$.


In the query phase, a pair query $u$, $v$ is answered in two steps.
\begin{compactenum}
\item For the LCA bag $\PNode{\Bag}$ of $\PNode{\Bag}_{u}$, $\PNode{\Bag}_{v}$,
and every partial node $\PNode{x}\in \PNode{\Bag}$, the distances $\Distance(u, \PNode{x})$
and $\Distance(\PNode{x}, v)$ are computed using the maps $\From$ and $\To$
along the paths $\PNode{\Bag}_{u}\Path \PNode{\Bag}$ and $\PNode{\Bag}\Path \PNode{\Bag}_{v}$ respectively.
\item Return $\bigoplus_{\PNode{x}\in \PNode{\Bag}} \Distance(u, \PNode{x})\otimes \Distance(\PNode{x}, v)$.
\end{compactenum}

It follows easily from \cref{lem:preproces_complexity} and the above modification
that the preprocessing time is $O(n^3)$.
The query time is $O(|\PNode{\Bag}|\cdot (|\PNode{\Bag}_1| + \PNode{\Bag}_2|))=O(n^2)$, where $\PNode{\Bag}_1$ and $\PNode{\Bag}_2$
are the children of the LCA $\PNode{\Bag}$ on the paths $\PNode{\Bag}_{u}\Path\PNode{\Bag}$ and $\PNode{\Bag}\Path\PNode{\Bag}_{v}$ respectively.



\smallskip\noindent{\bf Informal description of $\ConcurAP^{\eps}$.}
We are now ready to describe the modifications in obtaining $\ConcurAP^{\eps}$.
In order to answer a pair query in $O(n^{2-\eps})$ time,
we need to be able to recover the distances $\Distance(u, \PNode{x})$
and $\Distance(\PNode{x}, v)$ faster.
This is achieved by choosing two appropriate values: (i)~$\ell$ that depends on $\eps$ and $n$, and (ii)~$\lambda\in \Nats$,
and splitting $\PNode{T}$ into smaller subtrees $\PNode{T}_i$, every $\lambda\cdot \ell$ levels.
Then, the maps $\From_{u}$ and $\To_{u}$ of nodes $u$
store the distances between $u$ and partial nodes $\PNode{v}$ that appear in the ancestors of $\PNode{\Bag}_u$
which are in the same subtree $\PNode{T}_i$ as $\PNode{\Bag}_u$.
Afterwards, the distance between $u$ and every node $\PNode{x}\in \PNode{\Bag}$
will be retrieved by traversing the path $\PNode{\Bag}_u\Path \PNode{\Bag}$ in large steps of length $\lambda\cdot \ell$.
The time complexity for this traversal is again
$O(|\PNode{\Bag}|\cdot (|\PNode{\Bag}_1| + \PNode{\Bag}_2|))$, where $\PNode{\Bag}$ is the LCA bag of $\PNode{\Bag}_u$ and $\PNode{\Bag}_v$. 
However, this time $\PNode{\Bag}_1$ and $\PNode{\Bag}_2$
are descendants of $\PNode{\Bag}$ appearing $\lambda\cdot \ell$ levels below (instead of children), and are polynomially smaller
than the children of $\PNode{\Bag}$.
\cref{fig:tradeoff} provides an illustration.

\input{fig_tradeoff}


\smallskip\noindent{\bf $\ConcurAP^{\eps}$ preprocessing.}
Let $\lambda=5$ and $\Logratio=\frac{3^\lambda}{2^{\lambda-1}}$, and $\ell=\eps\cdot \log_{\Logratio}n$.
The preprocessing for $\ConcurAP^{\eps}$ consists of the same steps as that of $\ConcurAP$, with the following modification.
Instead of the preprocessing in \cref{item:ancestors} of $\Concpreprocessalgo$ on the whole $\PNode{T}$,
we do the following:
\begin{compactenum}
\item Partition $\PNode{T}$ into a set of trees $\{\PNode{T}_r\}_r$ such that for each $\PNode{T}_r$ there exists a $i\in \Nats$ for which
(i) the root bag of $\PNode{T}_r$ is in level $i\cdot \lambda\cdot \ell$ of $\PNode{T}$, and 
(ii) every other bag of $\PNode{T}_r$ is at most in level $(i+1)\cdot \lambda\cdot \ell$ of $\PNode{T}$.
\item Preprocess each $\PNode{T}_r$ according to \cref{item:ancestors} of $\Concpreprocessalgo$.
\end{compactenum}
Note that besides the root bag of $\PNode{T}$, 
the root bag of every tree $\PNode{T}_r$ is a leaf in some other 
tree $\PNode{T}_{r'}$. In such a case we call $\PNode{T}_{r'}$ the
\emph{parent tree} of $\PNode{T}_r$. 
For some $i\in \Nats$, we say that a tree $\PNode{T}_r$ constructed this way \emph{appears in the $i$-th level},
if the root of $\PNode{T}_r$ appears in the level $i\cdot \lambda\cdot \ell$ of $\PNode{T}$.




\smallskip
\begin{lemma}\label{lem:eps_preprocess_correctness}
The preprocess phase of $\ConcurAP^{\eps}$ requires $O(n^{3+\eps})$ time
and $O(n^{2.4})$ space.
\end{lemma}
\begin{proof}
We analyze the time and space required for the modified preprocessing.
We first focus on the space requirement. 
For any $i\in \Nats$, consider any tree $\PNode{T}_r$ that appears in level $i$,
and node $u$ such that $\PNode{\Bag}_u$ is a bag of $\PNode{T}_r$.
It follows from the analysis of \cref{item:ancestors} of \cref{lem:preproces_complexity}
that $\AncestV{\PNode{V}}_{\PNode{T}_r}(\PNode{\Bag}_u)=O(n\cdot 2^{-(\lambda-1)\cdot i\cdot \ell})$.
In view of \cref{rem:bag_size}, 
the space required for storing the maps $\From_u$ and $\To_u$ for all nodes $u$ whose root bag $\PNode{\Bag}_u$
appears in a tree $\PNode{T}_r$ of level $i$ is given by the following recurrence, up to a constant factor.
\begin{align*}
\Space(i) & \leq n\cdot 2^{-(\lambda-1)\cdot i\cdot \ell} \cdot \sum_{j=(i+1)\cdot \ell}^{i\cdot \ell} \left(3^{\lambda \cdot j}\cdot n\right)\\
&\leq n^2\cdot 2^{-(\lambda-1)\cdot i\cdot \ell} \cdot 3^{\lambda\cdot(i+1)\cdot \ell}\\
&\leq n^2 \cdot R^{i\cdot \ell}\cdot 3^{\lambda\cdot \ell}
\leq n^{2 + i\cdot \eps}\cdot 3^{\lambda\cdot \ell}
%&\leq n^{2+\frac{\eps\cdot (\lambda-1)}{\log \Logratio}} \leq n^{2+1.02\cdot \eps}
\end{align*}
since $\Logratio=\frac{3^{\lambda}}{2^{\lambda-1}}$ and $\ell=\eps\cdot \log n$.
Thus $S(i)=o(S(i+1))$, and the space usage is dominated by the trees $\PNode{T}_r$
that appear in the maximum possible level $i^{*}$ of $\PNode{T}$.
It can be verified that there exists a constant $c$ such that the space usage of the trees in the maximum level is
bounded by
\[
S(i^*)\leq c\cdot n^{2+\frac{\eps\cdot (\lambda-1)}{\log \Logratio}} \leq c\cdot n^{2+1.02\cdot \eps}
\]
since $\frac{\lambda-1}{\log \Logratio}<1.02$.
As $\eps\in[0, \Epsbound]$, we have $\Space(i^{*})=O(n^{2.4})$.
Since the other steps of the preprocessing of $\ConcurAP^{\eps}$
are given by the algorithm $\Concpreprocessalgo$,
in combination with \cref{lem:preproces_complexity} we obtain that the space usage of the preprocessing for $\ConcurAP^{\eps}$
is $O(n^{2.4})$.

Similarly, the time required for computing the maps $\From_u$ and $\To_u$ for all nodes $u$ whose root bag $\PNode{\Bag}_u$
appears in a tree $\PNode{T}_r$ of level $i$ is given by the following recurrence (again, we ignore constant factors).
\begin{align*}
\Time(i) & \leq n\cdot 2^{-(\lambda-1)\cdot i\cdot \ell} \cdot \sum_{j=(i+1)\cdot \ell}^{i\cdot \ell}
\left(\left(\frac{3^\lambda}{2^{\lambda-1}}\right)^j \cdot n^2\right)\\
& \leq \cdot n^3 \cdot 2^{-(\lambda-1)\cdot i\cdot \ell} \cdot \left(\frac{3^\lambda}{2^{\lambda-1}}\right)^{(i+1)\cdot \ell}\\
& \leq \cdot n^3\cdot \left(\frac{3^{\lambda}}{2^{2\cdot(\lambda-1)}}\right)^{i\cdot \ell}\cdot \left(\frac{3^{\lambda}}{2^{\lambda-1}}\right)^{ \ell}\\
&\leq \cdot n^{3}\cdot R^{\ell} = O(n^{3+\eps})
\end{align*}
In combination with \cref{lem:preproces_complexity}, the desired result follows.
\end{proof}


\smallskip\noindent{\bf $\ConcurAP^{\eps}$ query.}
The single-source and partial pair queries in for which both nodes are strictly partial
(\cref{item:ss_query} and \cref{item:spp_query} of $\Concqueryalgo$ respectively)
are handled in the same way as in $\ConcurAP$. 
Here we describe the remaining cases.
\begin{compactenum}
\item \emph{Pair query.} Given two nodes $u,v\in V$, find the LCA $\PNode{\Bag}$ of bags $\PNode{\Bag}_u$ and $\PNode{\Bag}_v$.
If the bags $\PNode{\Bag}_u$ and $\PNode{\Bag}_v$ are in the same tree $\PNode{T}_i$,
return $\bigoplus_{x\in \PNode{\Bag}\cap V} (\From_u(x) \otimes \To_v(x))$.
Else, assume w.l.o.g. that $\PNode{\Bag}_u$ and $\PNode{\Bag}$ are in trees $\PNode{T}_i$ and $\PNode{T}_{i'}$
respectively, with $i\neq i'$, and let $\PNode{\Bag}^i$ be the root of $\PNode{T}_i$.
For every node $x\in \PNode{\Bag}^i\cap V$, obtain the distance $\Distance(x,v)$ recursively.
Return $\bigoplus_{x\in \PNode{\Bag}^i\cap V} \From_u(x) \otimes \Distance(x,v)$.
\item  \emph{Partial pair query.} Given two partial nodes $\PNode{u}, \PNode{v}$ where exactly one is strictly partial,
the query is answered similarly as the pair query, with the restriction that the LCA bag is the root of $\PNode{T}$,
and only the non-partial node can have its root bag in some $\PNode{T}_i$ whose root is not the root of $\PNode{T}$.
\end{compactenum}



\smallskip
\begin{theorem}\label{them:tradeoff}
Let $G=(V,E)$ be a concurrent graph of two constant-treewidth graphs $G_1, G_2$,
$\Weight:E\to \Sigma$ a weight function of $G$
and $\eps\in [0,\Epsbound]$.
The data-structure $\ConcurAP^{\eps}$ correctly answers single-source and pair queries and requires:
\begin{compactenum}
\item Preprocessing time $O(n^{3+\eps})$
\item Preprocessing space $O(n^{2.4})$
\item Single-source query time $O(n^{2.4})$
\item Pair  query time $O(n^{2-\eps})$
\item Partial pair query time $O(n^{2-3\cdot \eps})$.
\end{compactenum} 
\end{theorem}
\begin{proof}
The correctness follows immediately from \cref{lem:preprocess_correctness},
and the time and space complexity for preprocessing is given in \cref{lem:eps_preprocess_correctness}.
Let $\Time(u,v)$ be the time to answer a pair query between nodes $u$ and $v$.
In view of \cref{rem:bag_size}, the time spent to traverse 
from the root $\PNode{\Bag}_{i+1}$ of a tree $\PNode{T}_{i+1}$ at level $(i+1)\cdot\lambda\cdot \ell$ to the root $\PNode{\Bag}_{i}$ of its parent $\PNode{T}_{i}$ at level $i\cdot\lambda\cdot \ell$
is 
\[
O\left(|\PNode{\Bag}_{i+1}|\cdot |\PNode{\Bag}_{i}|\right)=O\left(n^2\cdot 2^{-(\lambda-1)\cdot (2\cdot i + 1) \cdot \ell}\right)
\]
as for all $j$ and root bags $\PNode{\Bag}_j$ of trees $\PNode{T}_j$ at level $j$
we have $|\PNode{\Bag}_{j}| = O(n\cdot 2^{-j\cdot (\lambda-1)\cdot \ell})$.
Summing over all such levels, we obtain (ignoring constant factors)
\begin{align*}
\Time(u,v) &\leq \sum_{i=0}^{h} \left(n^2\cdot 2^{-(\lambda-1)\cdot (2\cdot i + 1) \cdot \ell}\right)\\
& = n^2\cdot 2^{-(\lambda-1)\cdot \ell}\cdot \sum_{i=0}^{h} \left(2^{-2\cdot i\cdot (\lambda-1)\cdot \ell}\right)\\
& \leq c\cdot n^2\cdot 2^{-(\lambda-1)\cdot \eps\cdot \log_{\Logratio} n}\\
& = c\cdot n^{2-\eps \cdot \frac{\lambda-1}{\log R}}\leq c\cdot n^{2-\eps}
\end{align*}
since $\frac{\lambda-1}{\log_{\Logratio}n} > 1$. Hence we have $\Time(u,v)=O(n^{2-\eps})$.

Finally, we consider a partial pair query between nodes $\PNode{u}$ and $\PNode{v}$, where at least one is strictly partial.
The corresponding time $\Time(\PNode{u}, \PNode{v})$ is given by a similar recurrence, but this time $i$ runs from $1$,
as at least one of $\PNode{u}$ and $\PNode{v}$ appears in the root of $\PNode{T}$.
\[
\Time(\PNode{u},\PNode{v}) \leq \sum_{i=1}^{h} \left(n^2\cdot 2^{-(\lambda-1)\cdot (2\cdot i + 1) \cdot \ell}\right)\\
\]
It can be verified that $\Time(\PNode{u}, \PNode{v}) = O(n^{2-3\cdot \eps})$.
The desired result follows.
\end{proof}


==> tree_decomposition_old.tex <==
\section{Construction of a $(\Bagfactor,\Balfactor,\Levelfactor)$ tree-decomposition}\label{sec:tree_decomp}

In this section we show how given a graph $G$
and a tree-decomposition $\Tree(G)$ of $b$ bags and width $t$,
we can construct in $O(b\cdot \log b)$ time and $O(b)$ space a $(\Bagfactor, \Balfactor, \Levelfactor)$ tree-decomposition with $b$ bags.
That is, the resulting tree-decomposition has width at most $\Bagfactor \cdot (t+1)$, 
and for every bag $\Bag$ and descendant $\Bag'$ of $\Bag$ $\Levelfactor$ levels below,
$|T(\Bag')|\leq \Balfactor\cdot |T(\Bag)|$ (i.e., the number of bags in $T(\Bag')$ is at most $\Balfactor$ times
as large as that in $T(\Bag)$).
The result is established in two steps.
First, we arrange the bags of $\Tree(G)$ to a ternary \emph{rank tree} $\Ranktree$ of $G$ such that every bag of $\Ranktree$
is $(\Balfactor, \Levelfactor)$-balanced.
Then, we show how to turn $\Ranktree$ to a $(\Bagfactor)$-approximate tree-decomposition $\widehat{\Ranktree}$
by a simple modification.

\smallskip\noindent{\bf Operation $\Mergealgo$.}
Consider a forest of trees $\mathcal{T}=(T_1,\dots T_k)$, and let $|\mathcal{T}|=\sum_i |T_i|$
where $|T_i|$ is the number of nodes in $T_i$.
Let $j$ be the largest integer such that $\sum_{i=1}^j|T_i|\leq \frac{|\mathcal{T}|}{2}$.
We define the operation $\Mergealgo(\mathcal{T})=(\mathcal{T}_1, \mathcal{T}_2)$,
where $\mathcal{T}_1=(T_1,\dots, T_j)$ and $\mathcal{T}_2=(T_{j+1},\dots, T_k)$.
The following claim follows immediately.

\smallskip
\begin{claim}\label{claim:merge}
If $|T_i|<\frac{\delta}{2}\cdot |\mathcal{T}|$ for all $1\leq i\leq k$, then $|\mathcal{T}_1|\leq |\mathcal{T}_2|\leq \frac{1+\delta}{2}\cdot |\mathcal{T}|$.
\end{claim}



\smallskip\noindent{\bf Construction of the rank tree}.
In the following, we consider that $T_G=\Tree(G)=(V_T, E_T)$ is binary
and has $|V_T|=b$ bags. A \emph{connected component} of $\Tree(G)$ is a set of bags $\Comp\subseteq V_T$
that form a subtree of $\Tree(G)$. The \emph{neighborhood} $\Nhood(\Comp)$ of $\Comp$
is the set of bags in $V_T\setminus \Comp$ that have a neighbor in $\Comp$, i.e.
\[
\Nhood(\Comp) = \{\Bag\in V_T\setminus \Comp:~(\{\Bag\}\times \Comp)\cap E_T\neq \emptyset\}
\]

Given $T_G$, we assign to each bag $\Bag\in V_T$
a rank $\Rank(\Bag)\in \Nats$ according to the following recursive algorithm $\Rankalgo$.
Initially, we assign $\Rank(\Bag)=\bot$ for every bag $\Bag\in V_T$.
$\Rankalgo$ takes a fixed parameter $\lambda\in \Nats$, with $\lambda\geq 2$, 
and operates recursively on inputs $(\Comp, \ell, k)$ where $\Comp$ is a connected component of $T_G$,
$\ell\in \{0\}\cup [\Levelfactor-1]$,
and $k\in \Nats$ is the rank to be assigned, as follows.
\begin{compactenum}
\item If $\Comp$ contains a single bag $\Bag$, assign $\Rank(\Bag)=k$ and terminate. 
%%Otherwise,
\item\label{item:spliC1} Else, if $\ell> 0$, find a bag $\Bag$ whose removal splits $\Comp$ into connected components $\Comp_1,\Comp_2,\Comp_3$
with $|\Comp_i|\leq \frac{|\Comp|}{2} $ for each $i\in \Children$.
Assign $\Rank(\Bag)=k$, and call $\Rankalgo$ recursively on input $(\Comp_i, (\ell+1)\mod \Levelfactor, k+1)$ for each connected
component $(\Comp_i)_{1\leq i\leq 3}$.
\item\label{item:spliC2} Else, if $\ell=0$,
find a bag $\Bag$ whose removal splits $\Comp$ into connected components $\Comp_1,\Comp_2,\Comp_3$
with $|\Nhood(\Comp_i)\cap \Nhood(\Comp)|\leq \frac{\Nhood\Comp}{2}$ for each $i\in \Children$.
Assign $\Rank(\Bag)=k$, and call $\Rankalgo$ recursively on input $(\Comp_i, (\ell+1)\mod \Levelfactor , k+1)$
for each component $(\Comp_i)_{1\leq i\leq 3}$ created from $\Comp$ by removing $\Bag$.
Else,  call $\Rankalgo$ recursively on input $(\Comp, \ell, k)$.
\end{compactenum}


When \cref{item:spliC1} or \cref{item:spliC2} apply, we call the bag $\Bag$ a \emph{separator} of the component $\Comp$.
\cref{fig:nhood} illustrates the recursive step of the algorithm.
Algorithm $\Rankalgo$ induces a ternary \emph{rank tree} $\Ranktree$ of $G$ such that
the root is the unique bag $\Bag$ with $\Rank(\Bag)=0$, and a bag $\Bag'$ is 
the $i$-th child of a bag $\Bag$ iff $\Bag'$ is the separator of 
the sub-component $\Comp_i$ of the component $\Comp$
of which $\Bag$ is a separator. The level $i$ of $\Ranktree$ contains all bags $\Bag$ with
$\Rank(\Bag)=i$. 
The bags of $\Ranktree$ are exactly the bags of $T_G$.
To distinguish between various trees,
given a tree of bags $T$ (e.g. $\Ranktree$ ) and pair of bags $\Bag_1$, $\Bag_2$, we write
$\Bag_1\Path_{T}\Bag_1$ to denote
the unique acyclic path from $\Bag_1$ to $\Bag_2$ in $T$.


Given the rank function $\Rank$, we define the \emph{neighborhood} of a bag $\Bag$ as
\begin{align*}
\Nhood(\Bag) &= \{\Bag'\in V_T:\Rank(\Bag')< \Rank(\Bag) \text{ and for all intermediate bags}\\
&\Bag'' \text{ in the path } \Bag\Path_{T_G} \Bag',~\Rank(\Bag)\leq \Rank(\Bag'')\}\\
\end{align*}

i.e, $\Nhood(\Bag)$ consists of the bags $\Bag'$ that have smaller rank than $\Bag$, 
and that $\Bag$ can reach through a path that traverses intermediate bags of larger rank.
The following observations are straightforward. 

\smallskip
\begin{remark}\label{rem:nhoods}
For any component $\Comp$ examined by $\Rankalgo$ and $\Bag$ chosen as a separator of $\Comp$,
we have $\Nhood(\Bag)=\Nhood(\Comp)$.
\end{remark}


\smallskip
\begin{remark}\label{prop:nhood_parent}
Let $\Bag$ and $\Bag'$ be respectively a bag and its parent in $\Ranktree$. 
Then $\Nhood(\Bag)\subseteq \Nhood(\Bag')\cup\{\Bag'\}$,
and thus $|\Nhood(\Bag)|\leq |\Nhood(\Bag')|+1$.
\end{remark}

\input{fig_nhood}

Since every bag in $\Ranktree$ corresponds to a bag in $\Tree(G)$, the bags of $\Ranktree$ already cover all nodes and
edges of $G$ (i.e., properties C1 and C2 of a tree-decomposition).
In the following we show how $\Ranktree$ can be modified to also satisfy condition C3,
i.e., that every node $u$ appears in a contiguous subtree of $\Ranktree$.
Given a bag $\Bag$, we denote by $\Nhoodnodes(\Bag)=\Bag\cup \bigcup_{\Bag'\in \Nhood(\Bag)}\Bag'$,
i.e., $\Nhoodnodes(\Bag)$ is the set of nodes of $G$ that appear in $\Bag$ and its neighborhood.
In \cref{lem:gap} we will show the crucial property that for every pair of bags $\Bag_1$ and $\Bag_2$ such that 
$\Bag_1$ is ancestor of $\Bag_2$ in $\Ranktree$, every node $u\in (\Bag_1\cap\Bag_2)$ is in the neighborhood $\Nhoodnodes(\Bag)$
of every bag $\Bag$ of the path $\Bag_1\Path_{\Ranktree} \Bag_2$.
We start with a basic claim that will be useful throughout this section.

\smallskip
\begin{claim}\label{claim:lca}
For all $\Bag_1,\Bag_2\in V_T$, let $\Bag$ be their LCA in $\Ranktree$ and $P$ be the unique acyclic path $\Bag_1\Path_{T_G} \Bag_2$. 
Then $\Bag\in P$ and all $\Bag'$ in $P$ are descendants of $\Bag$ in $\Ranktree$.
\end{claim}
\begin{proof}
Let $\Comp$ be the smallest component processed by $\Rankalgo$ that contains both $\Bag_1$ and $\Bag_2$.
Then $\Bag$ was chosen as a separator for $\Comp$, hence $\Bag\in P$, and by the recursion,
all $\Bag'$ in $\Bag_1\Path_{T_G} \Bag_2$ will be descendants of $\Bag$ in $\Ranktree$. 
\end{proof}


We say that a pair of bags $(\Bag_1$, $\Bag_2)$ \emph{form a gap} of some node $u$ in a tree $T$ of bags (e.g., $\Ranktree$)
if $u\in \Bag_1\cap \Bag_2$
and for the unique acyclic path $P:\Bag_1\Path_T \Bag_2$ we have that $|P|\geq 2$ (i.e., there is at least one intermediate bag in $P$)
and for all intermediate bags $\Bag$ in $P$ we have $u\not\in \Bag$.

\smallskip
\begin{lemma}\label{lem:gap}
For every node $u$, and pair of bags $(\Bag_1$, $\Bag_2)$ that form a gap of $u$ in $\Ranktree$, such that $\Bag_1$ is an ancestor of $\Bag_2$,
for every intermediate bag $\Bag$ in $P:\Bag_1\Path_{\Ranktree} \Bag_2$ in $\Ranktree$, 
we have that $u\in \Nhoodnodes(\Bag)$.
\end{lemma}
\begin{proof}
The proof is by showing that $\Bag_1\in\Nhood(\Bag)$.
Fix arbitrarily such a bag $\Bag$, and since $\Bag$ is ancestor of $\Bag_2$ we have that $\Rank(\Bag)<\Rank(\Bag_2)$.
Let $P_1:\Bag\Path_{T_G} \Bag_2$ and $P_2:\Bag_2\Path_{T_G} \Bag_1$.
We argue that for all intermediate bags $\Bag'$ in $P_1$ and $P_2$, we have
that $\Rank(\Bag)<\Rank(\Bag')$.
When $\Bag'$ is an intermediate bag of $P_1$, the statement follows from Claim~\ref{claim:lca} 
since the LCA of $\Bag$ and $\Bag_2$ in $\Ranktree$ is $\Bag$.
Now consider that $\Bag'$ is an intermediate bag in $P_2$. From property C3 of a tree-decomposition,
since $u\in \Bag_1$ and $u\in \Bag_2$, then $u\in \Bag'$. Since $\Bag_1$ is the
LCA of $\Bag_1$ and $\Bag_2$ in $\Ranktree$, by Claim~\ref{claim:lca} $\Bag'$ is a descendant
of $\Bag_1$ in $\Ranktree$. Let $\Bag''$ be the LCA of $\Bag_2$ and $\Bag'$ in $\Ranktree$, and
$\Bag''$ is also a descendant of $\Bag_1$. By Claim~\ref{claim:lca}, $\Bag''$ is a node in the path
$P_3:\Bag_2\Path_{T_G} \Bag'$, hence $u\in \Bag''$. Since $(\Bag_1,\Bag_2)$ form
a gap of $u$, it follows that $\Bag''=\Bag_2$,
and $\Bag'$ is a descendant of $\Bag_2$, hence $\Rank(\Bag)<\Rank(\Bag_2)<\Rank(\Bag')$.

The above conclude that all intermediate nodes $\Bag'$ in the path $\Bag\Path_{T_G} \Bag_1$
have rank $\Rank(\Bag)<\Rank(\Bag')$, and since $\Rank(\Bag_1)<\Rank(\Bag)$, we have that $\Bag_1\in \Nhood(\Bag)$. 
Since, $u\in \Bag_1$ it is $u\in \Nhoodnodes(\Bag)$ and the desired result follows.
\end{proof}

%\input{fig_nhood}

\smallskip\noindent{\bf Turning the rank tree to a tree-decomposition.}
\cref{lem:gap} suggests a way to turn the rank tree $\Ranktree$ to a tree-decomposition.
Let $\widehat{\Ranktree}=\Rep(\Ranktree)$ be the tree obtained by replacing each bag $\Bag$ of $\Ranktree$ 
with $\Nhoodnodes(\Bag)$. 
For a bag $\Bag$ in $\Ranktree$ let $\widehat{\Bag}$ be the corresponding bag in $\widehat{\Ranktree}$ 
and vice versa.
The following lemma states that $\widehat{\Ranktree}$ is a tree-decomposition of $G$. 

\smallskip
\begin{lemma}\label{lem:balance_correctness}
$\widehat{\Ranktree}=\Rep(\Ranktree)$ is a tree-decomposition of $G$.
\end{lemma}
\begin{proof}
It is straightforward to see that the bags of $\widehat{\Ranktree}$ cover all nodes and edges of $G$
(properties C1 and C2 of the definition of tree-decomposition),
because for each bag $\Bag$, we have that $\widehat{\Bag}$ is a supserset of $\Bag$.
It remains to show that every node $u$ appears in a contiguous subtree of $\widehat{\Ranktree}$
(i.e., that property C3 is satisfied).
Assume towards contradiction otherwise, and it follows that there exist bags
$\widehat{\Bag}_1$ and $\widehat{\Bag}_2$ in $\widehat{\Ranktree}$ that form a gap of some node $u$ and let $\widehat{P}:\widehat{\Bag}_1\Path_{\widehat{\Ranktree}} \widehat{\Bag}_2$ be the path between them.
Observe that for any bag $\Bag$, if $u\not\in \Bag$, but $u\in \widehat{\Bag}$, then $u$ is also in the parent of $\widehat{\Bag}$, by Fact~\ref{prop:nhood_parent}. 
Hence, if $u\not\in (\Bag_1\cap\Bag_2)$, then $u$ is in a parent of either $\widehat{\Bag}_1$ or $\widehat{\Bag}_2$.

First we establish that one $\widehat{\Bag}_i$ must be ancestor of the other.
If not, let $\widehat{L}$ be the LCA of $\widehat{\Bag}_1$ and $\widehat{\Bag}_2$ in $\Ranktree$. Since $\widehat{L}\in\widehat{P}$, we get that $u\not\in \widehat{L}$. Hence, $u\not\in L$ and thus $u\not\in (\Bag_1\cap\Bag_2)$ by Claim~\ref{claim:lca} and property C3 of tree-decomposition. This indicates that $u$ is in a parent of either $\widehat{\Bag}_1$ or $\widehat{\Bag}_2$. But $\widehat{P}$ goes through both parents, contradicting that $\widehat{\Bag}_1$ and $\widehat{\Bag}_2$
form a gap.



Next, consider that $\widehat{\Bag}_1$ is an ancestor of $\widehat{\Bag}_2$ (the case where $\widehat{\Bag}_1$ is a descendant of $\widehat{\Bag}_2$ is symmetric). Observe that $u\not\in (\Bag_1\cap \Bag_2)$, since otherwise we get a contradiction from \cref{lem:gap}.
We have that $u\in \Bag_2$, since otherwise  $u$ also appears in the parent of $\widehat{\Bag}_2$, which is in $\widehat{P}$. Hence we have that $u\not\in \Bag_1$. 
Let bag $\Bag'\in\Nhood(\Bag_1)$ be such that $u\in \Bag'$, and let $L'$ be the LCA of $\Bag'$ and $\Bag_2$ in $\Ranktree$.
It follows that $L'$ is an ancestor of $\Bag_1$.
By Claim~\ref{claim:lca}, $L'$ appears in the path $\Bag'\Path_{T_G} \Bag_2$, and hence, by property C3 of tree-decomposition
we have that $u\in L'$.
Let $\Bag''$ be the first bag in the path $\Bag_1\Path_{\Ranktree} L'$ that contains $u$.
Observe that $u$ does not appear in any intermediate bag of the path $P:\Bag_1\Path_{\Ranktree} \Bag_2$, because otherwise it contradicts that $\widehat{\Bag}_1$ and $\widehat{\Bag}_2$ form a gap of $u$.
Hence, $u$ does not appear in any intermediate bag of the path $P':\Bag''\Path_{\Ranktree} \Bag_1\Path_{\Ranktree} \Bag_2$,
thus $\Bag''$ and $\Bag_2$ form a gap of $u$ in $\Ranktree$.
By \cref{lem:gap}, for each $\Bag$ in $P'$, and thus especially for the ones in $P$, we have that $\widehat{\Bag}$ contains $u$,
contradicting that $\widehat{\Bag}_1$ and $\widehat{\Bag}_2$ form a gap of $u$.
The desired result follows.
\end{proof}


\smallskip\noindent{\bf Properties of the tree-decomposition $\widehat{\Ranktree}$.}
\cref{lem:balance_correctness} states that $\widehat{\Ranktree}$ obtained by replacing each bag of $\Ranktree$
with $\Nhoodnodes(\Bag)$ is a tree-decomposition of $G$. 
The remaining of the section focuses on showing that $\widehat{\Ranktree}$ is a $(\Bagfactor, \Balfactor, \Levelfactor)$
tree-decomposition of $G$, and that it can be constructed in $O(b\cdot \log  b)$ time and $O(b)$ space.

\smallskip
\begin{lemma}\label{lem:rank_assertions}
The following assertions hold:
\begin{compactenum}
\item \label{item:rank} Every bag $\widehat{\Bag}$ of $\widehat{\Ranktree}$ is $(\Balfactor, \Levelfactor)$-balanced.
\item \label{item:nhood} For each bag $\widehat{\Bag}$ of $\widehat{\Ranktree}$, we have $|\widehat{\Bag}|\leq \Bagfactor\cdot (t+1)$.
\end{compactenum}
\end{lemma}
\begin{proof}
We prove each item separately.
\begin{compactenum}
\item Let $\Bag$ be the separator of a component $\Comp$ when $\Rankalgo$ was executed on input $(\Comp, \ell, k)$,
and note that the bags of $\Ranktree(\Bag)$ are exactly the bags of $\Comp$.
For every $\Levelfactor$ consecutive recursive steps of $\Rankalgo$,
at least $\lambda-1$ will break the input component $\Comp$ to $(\Comp_i)_{1\leq i\leq 3}$
with $|\Comp_i|\leq\frac{|\Comp|}{2}$.
It follows that for every $\Bag$ in $\Ranktree$ and $\Bag'$ a descendant of $\Bag$
$\Levelfactor$ levels below, we have $|\Ranktree(\Bag')|\leq  \Balfactor\cdot |\Ranktree(\Bag)|$,
and thus $\Bag$ is $(\Balfactor, \Levelfactor)$-balanced in $\Ranktree$, and hence also in $\widehat{\Ranktree}$.
\item It suffices to show that $|\Nhood(\Bag)|\leq 2\cdot \lambda-1$.
Assume towards contradiction otherwise.
Let $\Bag$ be the first bag that $\Rankalgo$ assigned a rank such that $|\Nhood(\Bag)|\geq 2\cdot \lambda$.
Let $\Bag'$ be the lowest ancestor of $\Bag$ in $\Ranktree$ that was assigned a rank from $\Rankalgo$ on some input $(\Comp, \ell, k)$
with $\ell=1$, and let $\Bag''$ be the parent of $\Bag'$ in $\Ranktree$.
It follows that $|\Nhood(\Bag')|\leq\lfloor\frac{|\Nhood(\Bag'')|}{2}\rfloor+1$.
Note that $\Bag'$ is at most $\lambda-1$ levels above $\Bag$ (as we allow $\Bag'$ to be $\Bag$).
By \cref{rem:nhoods} and \cref{prop:nhood_parent}, $|\Nhood(\Bag)|$
can increase by at most one from the parent of $\Bag$ in $\Ranktree$, hence $\Nhood(\Bag')\geq \lambda+1$.
The last two inequalities lead to $|\Nhood(\Bag'')|\geq 2\cdot \lambda$, which contradicts our choice of $\Bag$.
The desired result follows.
\end{compactenum}
\end{proof}



\smallskip\noindent{\bf A minimal example.}
\cref{fig:TreeG2Rank2BalTreeG} illustrates an example of $\widehat{\Ranktree}$ constructed out of a tree-decomposition $\Tree(G)$ for $\lambda=2$.
First, $\Tree(G)$ is turned into a  binary and balanced tree $\Ranktree$ and then into a binary and balanced tree $\widehat{\Ranktree}$. 
If the numbers are pointers to bags, such that $\Tree(G)$ is a tree-decomposition for $G$, then $\widehat{\Ranktree}$ is a binary and balanced tree-decomposition of $G$.

\input{fig_balance}

\smallskip
\begin{theorem}\label{them:balanced_tree_decomp}
Consider a graph $G$ and a tree-decomposition $\Tree(G)$ of $G$ with $b$ bags be given.
For any fixed $\delta>0$ and $\lambda\in \Nats$ with $\lambda\geq 2$,
a binary $\abc$ tree-decomposition of $G$ can be constructed in $O(b\cdot \log b)$ time
and $O(b)$ space.
\end{theorem}
\begin{proof}
\cref{lem:balance_correctness} and \cref{lem:rank_assertions} prove that the constructed $\widehat{\Ranktree}$ is a
$(\Bagfactor, \Balfactor, \Levelfactor)$ tree-decomposition of $G$.
The time and space complexity come from the construction of $\Ranktree$ by the recursion of $\Rankalgo$.
It can be easily seen that every level of the recursion processes disjoint components $\Comp_i$ of $\Tree(G)$ in $O(|\Comp_i|)$
time, thus one level of the recursion requires $O(b)$ time in total. There are $O(\log b)$ such levels,
since every $\Levelfactor$ levels, the size of each component has been reduced to at most a factor $\Balfactor$.
Hence the time complexity is $O(b\cdot \log b)$.
The space complexity is that of processing a single level of the recursion, hence $O(b)$.
\end{proof}


